Unsupervised Scale-consistent Depth and Ego-motion Learning from Monocular Video

Recent work has shown that CNN-based depth and ego-motion estimators can be learned using unlabelled monocular videos. However, the performance is limited by unidentified moving objects that violate the underlying static scene assumption in geometric image reconstruction. More significantly, due to lack of proper constraints, networks output scale-inconsistent results over different samples, i.e., the ego-motion network cannot provide full camera trajectories over a long video sequence because of the per-frame scale ambiguity. This paper tackles these challenges by proposing a geometry consistency loss for scale-consistent predictions and an induced self-discovered mask for handling moving objects and occlusions. Since we do not leverage multi-task learning like recent works, our framework is much simpler and more efficient. Comprehensive evaluation results demonstrate that our depth estimator achieves the state-of-the-art performance on the KITTI dataset. Moreover, we show that our ego-motion network is able to predict a globally scale-consistent camera trajectory for long video sequences, and the resulting visual odometry accuracy is competitive with the recent model that is trained using stereo videos. To the best of our knowledge, this is the first work to show that deep networks trained using unlabelled monocular videos can predict globally scale-consistent camera trajectories over a long video sequence.

==> wording.tex <==
groundtruth -> ground truth
Equ -> Eqn
over-fit -> overfit


HY remarks:
- should we explain more about the scale-inconsistency issue? It is clear to ourselves that there is a scale-inconssitency issue. However, haven't seen a session/paragraph for explaining the issue in details. i.e the fundamental cause of the issue. Readers might not be able to get the problem easily.
Previous work suffers from
the per frame scale-ambiguity issue, in that an actual metric
scaling of the camera translations is missing and only direction is known
% 
- Explain why single-scale performance is different from other work's result, especially "digging into self-supervised depth"
https://arxiv.org/pdf/1806.01260.pdf
